$^{22}$Na Activation Level Measurements of Fused Silica Rods in the LHC Target Absorber for Neutrals (TAN) Compared to FLUKA Simulations

The Target Absorbers for Neutrals (TANs) are located in a high-intensity radiation environment inside the tunnel of the Large Hadron Collider (LHC). TANs are positioned about $140$ m downstream from the beam interaction points. Seven $40$ cm long fused silica rods with different dopant specifications were irradiated in the TAN by the Beam RAte of Neutrals (BRAN) detector group during $p$+$p$ data taking from 2016 to 2018 at the LHC. The peak dose delivered to the fused silica rods was $18$ MGy. We report measurements of the $^{22}$Na activation of the fused silica rods carried out at the University of Illinois at Urbana-Champaign and Argonne National Laboratory. At the end of the irradiation campaign, the maximum $^{22}$Na activity observed was $A=21$ kBq$/{\rm cm^3}$ corresponding to a density, $\rho= 2.5\times 10^{12} /{\rm cm^3}$, of $^{22}$Na nuclei. FLUKA Monte Carlo simulations have been performed by the CERN FLUKA team to estimate $^{22}$Na activities for the irradiated BRAN rod samples. The simulations reproduce the $^{22}$Na activity profile measured along the rods, with a 35% underestimation of the experimental measurement results.

==> backup.tex <==
% @article{Transmission:2022,
%     author = "Yang, Sheng and others",
%     title = "{Optical Transmission Measurements of Fused Silica Irradiated at the CERN Large Hadron Collider}",
%     year = "Paper in preparation"
% }

%This helps to prevent overheating of the blade and quartz rod and also greatly reduces the spread radioactive quartz dust from BRAN cuts, minimizing the risk of exposure to saw operators and contamination of the working area. 
%The saw blade itself is a resin bond, diamond wafering blade with outer diameter of 4”, arbor diameter 0.5”, and thickness 0.015”.\\


%The saw used to cut the BRAN rods is a UKAM Smart Cut 6001 Precision Sectioning Saw. This saw has a 1/4 [hp] motor with variable speed from 400 rpm to 3,400 rpm and a 15” $\times$ 9” saw plane. 

 %On the bottom of the rod holder are two guide-legs which fit into two corresponding slots on either end of the saw plane during cutting. These legs allow the rod holder to be guided smoothly down the length of the saw plane towards the blade. Sometimes, depending on stability needs and the characteristic of a given rod holder, only 1 guide-leg is necessary and the 2$^{\text{nd}}$ leg is either removed or not attached at the outset.The rod to be cut is ‘loaded’ into the holding apparatus and secured with padded supports held tightly in place by 1/4”-20 socket-head screws. %The loaded and secured rod is guided smoothly towards the blade by a gravity-feeding system as a cut is made. The gravity-feeding system is comprised of standard weights attached to one end of a string, with the other end fastened to the guide rail system. \\
%Once the rod is secure in the holding apparatus, it is ready to be cut. The gravity-feeding weights are carefully attached one at a time while the operator holds the string to ensure the rod holder does not unexpectedly slide towards the blade unrestrained. Once the weights are loaded, the operator gently pulls on the string until the rod holder just begins to move towards the blade.Once the surface of the rod reaches the blade, it is important to ensure that the holder continues moving and does not become stuck when the blade first strikes the rod – this tends to cause unwanted scratch marks on the face of the cut. The operator continues to guide the rod slowly but steadily through the blade, making the entire cut in one motion as the blade slices through the full diameter of the rod without stopping.


The installed BRAN prototype was irradiated from 2016 to 2018 and experienced different beam configurations. One of the important configures is the crossing angle of the LHC beams, which affects directly the instantaneous luminosity and the byproduct distribution of the collision reactions. When two LHC beams approach each other near an interaction point (IP), the beams collide at an angle of a couple of hundred microradians to prevent encounters in the region where the two beams share the same vacuum chamber~\cite{evans2008lhc}. A small crossing angle increases the overlap area of the bunches, resulting in a higher luminosity. Conversely, the angle must be large enough to mitigate the long-range interactions between the electromagnetic fields generated by the beams. Long-range interactions decrease due to the loss of intensity experienced by the beams in the collisions.  By exploiting this effect, LHC scientists were able to decrease the crossing angle at IP1 and IP5 (CMS) from 160 $\mu$rad to 130 $\mu$rad between 2016 and 2017 runs~\cite{evans2008lhc, lhcnews2017crossing}.


The BRAN (Beam RAte of Neutrals) was used to
monitor and optimize the luminosity in the Target Absorbers for Neutrals (TANs), located at $\pm$ 140 m from interaction regions (IR), IR1 (ATLAS) and IR5 (CMS). To upgrade the BRAN for High-Luminosity Large Hadron Collider, a BRAN prototype was installed in the TANs during $p$+$p$ running in 2015 - 2018 (Run2). The BRAN prototype accommodated up to eight 40 cm long fused silica rods to act as Cherenkov radiators when exposed to the shower of particles generated in the TAN. The particle showers produce activated isotopes within the fused silica rods that comprise the detector.
In this paper, we report the measurement of the activation in fused silica rods from BRAN prototype and compare the measurements to the activation estimated by FLUKA MonteCarlo simulations. The fused silica rods' activation was measured by a high purity Germanium detector at the University of Illinois at Urbana-Champaign and a NaI(Tl) well-type detector at Argonne National Laboratory. The measurement results were calibrated by a customized volume Na-22 source with a 3.3\% activity uncertainty. 
%The volume source was used to keep the systematic of the calibration under control.
FLUKA simulations have been performed to estimate the specific isotope yields for these BRAN rod samples while taking the crossing angle into account. 
%The isotope yield estimated by FLUKA simulations were compared to activation measurements of BRAN rod samples. 
Our results on the induced activity measured in samples show the agreement in the shape of the activity profile with the simulation estimation. However, the relative difference of the isotope yield between measurement and the simulation varies from 60\% to 90\%.  All these results indicate that there is a significant discrepancy between simulation and data. The result of activation measurements could benchmark the simulation since the physics of nuclide interaction in TeV range might not be simulated accurately. 


%The comparison of the normalized FLUKA activation profile with the experimental measurements shows good agreement. The discrepancy in the absolute normalization was found to be lower than a factor of 2.  

%sample preparation section
\iffalse%------------------------- 

Specifications for the cutting apparatus used to produce the BRAN rod segments are given in Tab.~\ref{Tab:Cutting_specification}. All BRAN rod cutting was performed using a wet cut, meaning that the bottom edge of the saw blade was constantly submerged in a mixture of water and coolant. This technique was used in order to reduce the impact of temperature dependent annealing on future transmission measurements while also reducing the spread of silica dust. \begin{table}[ht]
\centering
\caption{Specifications for BRAN Rod Cutting Apparatus} 
\begin{tabular}{|l | c | c |}
\hline
Model number & UKAM Smart Cut 6001  \\
\hline 
RPM   &  3,400  \\
\hline 
Blade Material & Resin Bond, Diamond \\
\hline
Blade Thickness & 0.015” \\
\hline
\end{tabular}
\label{Tab:Cutting_specification} 
\end{table}


The rod holder assembly consists of a Nylon-12 3D-printed block with a 1 cm wide channel machined into its surface that houses the BRAN rod to be cut. Along the length on either side of the channel are pairs of screw holes which allow the rod to be fastened into the holding apparatus.
Immediately after the cut is made and dried, the weights of both the cut and the remaining uncut rod are recorded. Digital calipers are then used to measure the $i^{th}$ segment's maximum length ($L_{i}^{max}$) and minimum length ($L_{i}^{min}$) by rotating the segment 360$^{\circ}$ within the calipers. The remaining rod length, $L_{i}^{rem}$, was also recorded for later calculations. The average cut length for the $i^{th}$ segment, $L_{i}$, is then determined:
\begin{equation}
 L_{i}=\left(\dfrac{L_{i}^{max}+L_{i}^{min}}{2}\right).
  \label{eq:avg_l}
\end{equation}

Using data collected from both the BRAN rod cuts and the many test-cuts taken while calibrating the cutting setup, the average amount of rod material \textit{lost} per-cut has been calculated to be $70$mg. This material is into dust by the blade and dragged down into the fluid reservoir of the saw. 
\fi%------------------------- 


\begin{figure}[htbp!]
     \centering
     \includegraphics[keepaspectratio,scale=0.3]{FLUKA/figs/Dosage_profile_YZ.png}
     \caption{Dosage Y-Z profile in the BRAN prototype in 2016 (right) and 2017 (left) respectively. The crossing angle in each year has been included in the simulation, as is evident from the vertical shift in the maximum exposure position. The luminosity in 2016 and 2017 was 36.5 and 50 fb$^{-1}$, respectively.}
     \label{fig:Dosage_profile_YZ}
\end{figure}



% material composition table
\definecolor{mayablue}{rgb}{0.45, 0.76, 0.98}
\definecolor{lapislazuli}{rgb}{0.15, 0.38, 0.61}
\definecolor{meatbrown}{rgb}{0.9, 0.72, 0.23}
\definecolor{purpleheart}{rgb}{0.41, 0.21, 0.61}
\definecolor{pakistangreen}{rgb}{0.0, 0.4, 0.0}

\begin{table*}[ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{BRAN}       & \textbf{Irradiation}  & \textbf{Max. Exposure}    & \multirow{2}{*}{\textbf{Material}}    & \textbf{H$_{2}$}  & \textbf{OH} \\ 
\textbf{Position}   & \textbf{Period}       & [MGy]                    &                                       & [mol/cm$^{3}$]    & [ppm] \\ 
\hline
\hline 

\multirow{2}{*}{\textbf{Control}}    &  \multirow{2}{*}{None}    & \multirow{2}{*}{0}    & Spectrosil 2000   & \multirow{2}{*}{7.20e17}     & \multirow{2}{*}{1120} \\ 
                            &                           &                       & (High OH, Mid H$_{2}$) &                           &  \\ 
\hline

\cellcolor{black}        &  04/2016 -    & \multirow{2}{*}{18}    & Spectrosil 2000   & \multirow{2}{*}{7.20e17}      & \multirow{2}{*}{1120} \\ 
\multirow{-2}{*}{\cellcolor{black}\textbf{\textcolor{white}1}}   &   12/2018     &                       & (High OH, Mid H$_{2}$) &                               &  \\ 
\hline
\cellcolor{red}                                                 &  04/2016 -    & \multirow{2}{*}{10}      & Spectrosil 2000   & \multirow{2}{*}{7.20e17}      & \multirow{2}{*}{1120} \\ 
\multirow{-2}{*}{\cellcolor{red}\textbf{\textcolor{white}2}}   &   12/2017     &                           & (High OH, Mid H$_{2}$) &                               &  \\ 
\hline
\cellcolor{pakistangreen}                                                   &  04/2016 -    & \multirow{2}{*}{5}      & Spectrosil 2000   & \multirow{2}{*}{2.80e18}      & \multirow{2}{*}{1000} \\ 
\multirow{-2}{*}{\cellcolor{pakistangreen}\textbf{\textcolor{white}{3a}}}    &   12/2016     &                           & (High OH, High H$_{2}$) &                               &  \\ 
\hline
\cellcolor{mayablue}                                                &  04/2017 -    & \multirow{2}{*}{16}      & Spectrosil 2000   & \multirow{2}{*}{7.20e17}      & \multirow{2}{*}{1120} \\ 
\multirow{-2}{*}{\cellcolor{mayablue}\textbf{\textcolor{white}{3b}}} &   12/2018     &                           & (High OH, Mid H$_{2}$) &                               &  \\ 
\hline
\cellcolor{lapislazuli}                                                 &  04/2016 -    & \multirow{2}{*}{9}      & Spectrosil 2000   & \multirow{2}{*}{0}      & \multirow{2}{*}{1011} \\ 
\multirow{-2}{*}{\cellcolor{lapislazuli}\textbf{\textcolor{white}4}}   &   12/2017     &                           & (High OH, H$_{2}$ free) &                               &  \\                     
\hline
\cellcolor{meatbrown}                                               &  04/2016 -    & \multirow{2}{*}{8}      & Suprasil 3301   & \multirow{2}{*}{3.00e18}      & \multirow{2}{*}{15} \\ 
\multirow{-2}{*}{\cellcolor{meatbrown}\textbf{\textcolor{white}5}} &   12/2017     &                           & (Low OH, High H$_{2}$) &                               &  \\                     
\hline
\cellcolor{purpleheart}                                                 &  04/2016 -    & \multirow{2}{*}{17}        & Suprasil 3301   & \multirow{2}{*}{0}      & \multirow{2}{*}{14} \\ 
\multirow{-2}{*}{\cellcolor{purpleheart}\textbf{\textcolor{white}6}}   &   12/2018     &                           & (Low OH, H$_{2}$ free) &                               &  \\                     
\hline
\end{tabular}
\caption{Fused silica rod specifications. The number ID assigned to each rod corresponds to a given position in the detector, as shown in Fig.~\ref{fig:BRANSet}. Rods 3a and 3b occupied the same slot, but at different times.}
\label{tab:BRANrods}%referenced
\end{table*}



\iffalse
%ARIC STUFF

current order:
- estimation of count rate HPGe detector
- estimation of na22 activity
- material loss correction
- cooling correction

proposed order:
- setup related correction/assumptions: 
        acceptance
- material loss correction, cooling correction >    
        sample related corrections/assumptions section: 
        cooling, material loss, homogeneous activity
- estimation of na22 activity
- estimation of count rate HPGe detector
- estimation of count rate well-type detector

%BOTH
- estimation of na22 activity
- cooling correction
- material loss correction

%UIUC
- estimation of count rate HPGe detector

%ANL
- ??? estimation of count rate Well type detector ???

TODO - write intro that describes the whole sequence



\fi
